Capturing research literature attitude towards Sustainable Development Goals: an LLM-based topic modeling approach

The world is facing a multitude of challenges that hinder the development of human civilization and the well-being of humanity on the planet. The Sustainable Development Goals (SDGs) were formulated by the United Nations in 2015 to address these global challenges by 2030. Natural language processing techniques can help uncover discussions on SDGs within research literature. We propose a completely automated pipeline to 1) fetch content from the Scopus database and prepare datasets dedicated to five groups of SDGs; 2) perform topic modeling, a statistical technique used to identify topics in large collections of textual data; and 3) enable topic exploration through keywords-based search and topic frequency time series extraction. For topic modeling, we leverage the stack of BERTopic scaled up to be applied on large corpora of textual documents (we find hundreds of topics on hundreds of thousands of documents), introducing i) a novel LLM-based embeddings computation for representing scientific abstracts in the continuous space and ii) a hyperparameter optimizer to efficiently find the best configuration for any new big datasets. We additionally produce the visualization of results on interactive dashboards reporting topics' temporal evolution. Results are made inspectable and explorable, contributing to the interpretability of the topic modeling process. Our proposed LLM-based topic modeling pipeline for big-text datasets allows users to capture insights on the evolution of the attitude toward SDGs within scientific abstracts in the 2006-2023 time span. All the results are reproducible by using our system; the workflow can be generalized to be applied at any point in time to any big corpus of textual documents.

==> old_sdg_table.tex <==
\begin{table}
\begin{tabularx}{\textwidth}{lXXr}
\toprule
\textbf{Macroarea} & \textbf{SDG} & \textbf{Keywords} & \textbf{\#abst.} \\
\midrule

\multirow{5}{*}{\makecell[l]{Basic Human\\ Needs and \\Well-being}} & 1 No Poverty & 
\multirow{5}{=}{Poverty alleviation; Food security; Public health; Education access; Water quality; Sanitation infrastructure; Healthcare provision.} & 333,901\\
& 2 Zero Hunger &&\rightarrow 333,901\\
& 3 Good Health and Well-being &&\rightarrow 320,798\\
& 4 Quality Education &\\
& 6 Clean Water and Sanitation &\\
\midrule

\multirow{6}{*}{\makecell[l]{Environment\\ Sustainability}} & 7 Affordable and Clean Energy & 
\multirow{6}{=}{Renewable energy; Urban sustainability; Sustainable consumption; Climate change mitigation; Marine biodiversity; Ecosystem conservation; Energy efficiency.} & 399,922\\
& 11 Sustainable Cities and Communities && \rightarrow 368,284\\
& 12 Responsible Consumption and Production &&\rightarrow 339,949\\
& 13 Climate Action \\
& 14 Life Below Water \\
& 15 Life on Land \\
\midrule

\multirow{6}{*}{\makecell[l]{Economic \\Development \\and Employment}} 
& 8 Decent Work and Economic Growth &
\multirow{6}{=}{Economic growth; Innovation ecosystems; Infrastructure development; Entrepreneurship support; Industrialization strategies; Industrial Innovation; Labor market dynamics.} & 50,482 \\
& 9 Industry, Innovation, and Infrastructure &&\rightarrow 45,116\\
&&&\rightarrow 41,218\\
&&\\
\midrule

\multirow{4}{*}{\makecell[l]{Equality and \\Social Inclusion}} 
& 5 Gender Equality &
\multirow{4}{=}{Gender empowerment; Social equity; Inclusive policies; Women's rights; Minority rights; Income inequality; Social justice.} & 33,769\\
& 10 Reduced Inequality &&\rightarrow 31,380\\
&&&\rightarrow 25,017\\
&&\\
\midrule

\multirow{6}{*}{\makecell[l]{Global \\Partnerships \\and Peace}} & 16 Peace, Justice, and Strong Institutions &
\multirow{6}{=}{Legal institutions; International cooperation; Peace efforts; Sustainable development cooperation; Global governance; Justice systems; Multilateral agreements.} & 56,275\\
& 17 Partnerships for the Goals &&\rightarrow 48,287\\
&&&\rightarrow 56,275\\
&&\\
&&\\
\bottomrule
\end{tabularx}
\caption{Description of five macro areas grouping the SDGs.}
\label{tab:groups}
\end{table}
